Can a binary star host three giant circumbinary planets?

We investigate the orbital stability of a tilted circumbinary planetary system with three giant planets. The planets are spaced by a constant number ($\Delta$) of mutual Hill radii in the range $\Delta=3.4-12.0$ such that the period ratio of the inner pair is the same as the outer pair. A tilted circumbinary planetary system can be unstable even if the same system around a coplanar binary is stable. For an equal mass binary, we find that the stability of a three-planet system is qualitatively similar to that of a two-planet system, but the three-planet system is more unstable in mean motion resonance regions. For an unequal mass binary, there is significantly more instability in the three-planet system as the inner planets can undergo von-Zeipel-Kozai-Lidov oscillations. Generally in unstable systems, the inner planets are more likely to be ejected than the outer planets. The most likely unstable outcome for closely spaced systems, with $\Delta \lesssim 8$, is a single remaining stable planet. For more widely separated systems, $\Delta \gtrsim 8$, the most likely unstable outcome is two stable planets, only one being ejected. An observed circumbinary planet with significant eccentricity may suggest that it was formed from an unstable system. Consequently, a binary can host three tilted giant planets if the binary stars are close to equal mass and provided that the planets are well spaced and not close to a mean motion resonance.

==> response.tex <==
Dear Scientific Editor and Assistant Editor,

We thank the referee for the useful report that has improved the manuscript. We have thoroughly reviewed the referee’s comments and made several changes to the manuscript. Referee-prompted changes in the updated document are highlighted in bold text. Additional edits, clarifying our methodology and results, are included, but not highlighted. We hope that you are satisfied with the revised manuscript.

Sincerely,
Cheng Chen, Rebecca G. Martin & Chris J. Nixon.


1)The author should clearly provide the value of the semi-major axes of the binary in the manuscript, such as ‘taking a_b=1’. Actually, a_b also has an impact on the results. 

RESPONSE: We thank the referee for mentioning it. We added a sentence at the end of first paragraph of Sec. 2 to clearly define a_b = 1.0. 


2)  - p2, col 2, paragraph 4: Sec. 2.3 ==> Section 2.3, The same below. To maintain consistency, I suggest using 'Section' throughout in this paragraph.

RESPONSE: We have changed all Sec. into section in the draft.

3)  - p3, col 1, line 35: Table. 1. ==> Table 1. 
  - p3, col 1, line 46: Fig 1 shows... ==> Fig. 1
  - p3, col 2, line 21: ‘there is a vertical unstable belt around i_p = 170 degrees Further, the region...’ ==> A . is missing before ‘Further’.
  - p6, line 34 in Figure 4: ‘...from the stability maps in Fig.2.’ ==> Fig. 2.
  - p6, col 1, line 42: Fig 4 ==> Fig. 4
  - p6, col 1, line 60: In Fig 5, ==> Fig. 5,
- p8, col 2,  in Figure 6: Similar to Fig 2...==> Fig. 2

RESPONSE: Thanks for raising these typos. We have fixed all of them.


3) In addition, the text in some figures also lack spaces. such as in Figure 1.
   Model: T1(f_b =0.5, e_b =0.0) ==> T1 (f_b.... .  The same below (in Figure 2-3).
RESPONSE: We have added the space in the title of Figure 1-3. 


Assistant Editor's Comments:
Please ensure that all textual labels in figures are at least as large as the caption text; any smaller and they become too difficult to read. 

RESPONSE: Thanks for raising this issue. We have enlarged labels in Figure 3 to make it clear.
